Resource-Efficient and Self-Adaptive Quantum Search in a Quantum-Classical Hybrid System

Over the past decade, the rapid advancement of deep learning and big data applications has been driven by vast datasets and high-performance computing systems. However, as we approach the physical limits of semiconductor fabrication in the post-Moore's Law era, questions arise about the future of these applications. In parallel, quantum computing has made significant progress with the potential to break limits. Major companies like IBM, Google, and Microsoft provide access to noisy intermediate-scale quantum (NISQ) computers. Despite the theoretical promise of Shor's and Grover's algorithms, practical implementation on current quantum devices faces challenges, such as demanding additional resources and a high number of controlled operations. To tackle these challenges and optimize the utilization of limited onboard qubits, we introduce ReSaQuS, a resource-efficient index-value searching system within a quantum-classical hybrid framework. Building on Grover's algorithm, ReSaQuS employs an automatically managed iterative search approach. This method analyzes problem size, filters fewer probable data points, and progressively reduces the dataset with decreasing qubit requirements. Implemented using Qiskit and evaluated through extensive experiments, ReSaQuS has demonstrated a substantial reduction, up to 86.36\% in cumulative qubit consumption and 72.72\% in active periods, reinforcing its potential in optimizing quantum computing application deployment.

==> sections/background_old.tex <==
\section{BACKGROUND AND MOTIVATION}


In traditional computing, a bit, which serves as the fundamental unit of information, possesses two possible values - $0$ and $1$, existing within a deterministic logic state. Initially introduced by physicists, a bit can be represented by any physical system with two potential states. Examples include the two directions of magnetization in a magnetic storage device or the two distinct voltage levels within a circuit. Today, bits pervade the realm of computing and information science, forming the backbone of computer systems.

In contrast, the quantum bit, or qubit, acts as the foundational unit of information in quantum computing, paralleling the role of a bit in classical computing. However, unlike bits, qubits exist in a superposition of two states. The states of qubits need to be well-defined only when measured to obtain an output. These states can be represented as orthogonal vectors, illustrating the inherent difference between classical and quantum computing units.

\begin{equation} 
    |0\rangle=
    \begin{bmatrix}
    1\\
    0
    \end{bmatrix}
    \qquad
    |1\rangle=
    \begin{bmatrix}
    0\\
    1
    \end{bmatrix}   
\end{equation}

These two orthogonal vectors $|0\rangle$ and $|1\rangle$ can represent any 2d vectors. For example, there is a vector $|q_0\rangle$,
\begin{equation}
    |q_0\rangle=
    \begin{bmatrix}
    \frac{1}{\sqrt{2}}\\
    \frac{i}{\sqrt{2}}
    \end{bmatrix},
\end{equation}
Using $|0\rangle$ and $|1\rangle$, $|q_0\rangle$ can be rewritten in this form. 
\begin{equation}
    |q_0\rangle=\frac{1}{\sqrt{2}} |0\rangle +\frac{i}{\sqrt{2}} |1\rangle
\end{equation}
Therefore, any vector $|q\rangle$ can be rewritten in this form,
\begin{equation}
    |q\rangle=\alpha|0\rangle+\beta|1\rangle
\end{equation}
where
\begin{equation}
    |\alpha|^2+|\beta|^2=1
\end{equation}

These vectors such as $|q_0\rangle$ are called the statevectors of qubits. A statevector is represented as a linear combination of two states. It is not just $|0\rangle$ and not just $|1\rangle$. In quantum mechanics, this situation is called superposition.~\citep{thomas2022introduction}.


\subsection{Quantum Gates}
Similar to classical data which is manipulated and encoded using gates, quantum data is manipulated and encoded using quantum gates. Quantum gates can either perform a rotation about an axis or perform an operation on a qubit based on the value of another qubit. These are referred to as rotation gates and controlled gates respectively.

\subsubsection{Single-Qubit Gates}


A common type of single-qubit operations are the rotation gates. These gates perform qubit rotations by parameterized amounts. The generalized single-rotation gate $R$ is shown in matrix form in Equation \ref{eq:rotation_general}.

\begin{equation}
R(\theta,\phi)=\left[\begin{array}{cc}
\cos \frac{\theta}{2} & -ie^{-i\phi}\sin \frac{\theta}{2} \\
-ie^{-i\phi}\sin \frac{\theta}{2} & \cos \frac{\theta}{2}
\end{array}\right]
\label{eq:rotation_general}
\end{equation}

Three commonly-used special cases of this gate are the $R_{X}$, $R_{Y}$, and $R_{Z}$ gates. These gates represent rotations in the x, y, and z plane and are expressed in Equations \ref{eq:rx}, \ref{eq:ry}, and \ref{eq:rz}. $R_{X}$ and $R_{Y}$ can be thought of as special cases of the $R$ gate in which $\phi = 0$ and $\phi = \frac{\pi}{2}$ respectively. Therefore, $R_{X}(\theta)$ is a rotation about the x-axis by angle $\theta$ and $R_{Y}(\theta)$ is a rotation about the y-axis by angle $\theta$. The derivation of $R_{Z}$ from the general rotation gate is less straightforward and thus is not included here.


\begin{equation}
R_{X}(\theta)=\left[\begin{array}{cc}
\cos \frac{\theta}{2} & -i\sin \frac{\theta}{2} \\
-i\sin \frac{\theta}{2} & \cos \frac{\theta}{2}
\end{array}\right]=R(\theta,0)
\label{eq:rx}
\end{equation}



\begin{equation}
R_{Y}(\theta)=\left[\begin{array}{cc}
\cos \frac{\theta}{2} & -\sin \frac{\theta}{2} \\
\sin \frac{\theta}{2} & \cos \frac{\theta}{2}
\end{array}\right]=R(\theta,\frac{\pi}{2})
\label{eq:ry}
\end{equation}

\begin{equation}
R_{Z}(\theta)=\left[\begin{array}{cc}
e^{\frac{-i\theta}{2}} & 0 \\
0&e^{\frac{-i\theta}{2}}
\end{array}\right]
\label{eq:rz}
\end{equation}


\subsubsection{Hadamard Gate}

A fundamental gate of quantum computation is the Hadamard gate. It is a single-qubit gate puts a qubit into superposition as described in Section~\ref{super}. It can be expressed in matrix shown in equation~\ref{eq:hgate}. The $\frac{1}{\sqrt{2}}$ coefficient is due to the fact that the sum of the squares of the state amplitudes must add to 1, so each state has a probability of $\frac{1}{2}$ and an amplitude of $\frac{1}{\sqrt{2}}$.

\begin{equation}
H=\frac{1}{\sqrt{2}}\left[\begin{array}{cc}
1 & 1 \\
1 & -1
\end{array}\right]
\label{eq:hgate}
\end{equation}



\subsubsection{Two-Qubit Gates}

There are also operations that function as two-qubit rotations which perform an equal rotation on two qubits. These gates are described in Equations \ref{eq:rxx}, \ref{eq:ryy}, and \ref{eq:rzz}. Note that these gates are expressed as 4x4 matrices while the single-qubit gates were 2x2 matrices. This is because for a two-qubit gate, each individual qubit has two possible measurements, yielding four possible results ($|00\rangle$,$|01\rangle$,$|10\rangle$,$|11\rangle$) rather than two as seen previously for the single-qubit gates.

\begin{small}
\begin{equation}
R_{XX}(\theta)=\left[\begin{array}{cccc}
\cos \frac{\theta}{2} & 0 & 0 & -i\sin \frac{\theta}{2}\\
0 & \cos \frac{\theta}{2} & -i\sin \frac{\theta}{2} & 0 \\
0 & -i\sin \frac{\theta}{2} & \cos \frac{\theta}{2} & 0 \\
-i\sin \frac{\theta}{2} & 0 & 0 & \cos \frac{\theta}{2}
\end{array}\right]
\label{eq:rxx}
\end{equation}
\end{small}

\begin{small}
\begin{equation}
R_{YY}(\theta)=\left[\begin{array}{cccc}
\cos \frac{\theta}{2} & 0 & 0 & i\sin \frac{\theta}{2}\\
0 & \cos \frac{\theta}{2} & -i\sin \frac{\theta}{2} & 0 \\
0 & -i\sin \frac{\theta}{2} & \cos \frac{\theta}{2} & 0 \\
i\sin \frac{\theta}{2} & 0 & 0 & \cos \frac{\theta}{2}
\end{array}\right]
\label{eq:ryy}
\end{equation}
\end{small}

\begin{small}
\begin{equation}
R_{ZZ}(\theta)=\left[\begin{array}{cccc}
e^{-i\frac{\theta}{2}} & 0 & 0 & 0\\
0 & e^{-i\frac{\theta}{2}} & 0 & 0 \\
0 & 0 & e^{-i\frac{\theta}{2}} & 0 \\
0 & 0 & 0 & e^{-i\frac{\theta}{2}}
\end{array}\right]
\label{eq:rzz}
\end{equation}
\end{small}

\subsubsection{Controlled Gates}

There are also two-qubit gates which utilize a control qubit and a target qubit. These gates, known as controlled gates, perform an operation on a target qubit depending on the value of the control qubit. 

{\bf \noindent CNOT Gate}
The CNOT gate is an example of a two-qubit gate used in quantum computing. The CNOT gate flips the value of the target qubit if the control qubit is measured as 1 and does nothing otherwise. The CNOT gate can be seen represented in matrix form below. 

\begin{equation}
CNOT=\left[\begin{array}{cccc}
1 & 0 & 0 & 0 \\
0 & 0 & 0 & 1 \\
0 & 0 & 1 & 0 \\
0 & 1 & 0 & 0
\end{array}\right]
\label{eq:squ-3}
\end{equation}

Fig.\ref{fig:cnot_gate} depicts the circuit notation for the CNOT gate. $q_{0}$ is the control qubit and $q_{1}$ is the target qubit.


%\begin{figure}[ht]			% Add figure one
%	\centering
%	\includegraphics[width=0.3\linewidth]{figures/cnot_gate2.png}
 %   \caption{CNOT Gate Circuit Notation}
 %   \label{fig:cnot_gate}
%\end{figure}

{\bf \noindent Controlled Rotation Gates}
Equations \ref{eq:crx}, \ref{eq:cry} and \ref{eq:crz} are controlled rotation gates in matrix notation. Controlled rotation gates are similar to the CNOT gate but apply a rotation when the control qubit measures 1 instead of flipping the state. This allows for variable levels of entanglement between qubits.

\begin{equation} 
\centering
CR_X(\theta)=\left[\begin{array}{cccc} 
1 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 \\
0 & 0 & \cos\frac{\theta}{2} & -\sin\frac{\theta}{2} \\
0 & 0 & -\sin\frac{\theta}{2} & \cos\frac{\theta}{2} 
\end{array}\right]
\label{eq:crx}
\end{equation}



\begin{equation} 
\centering
CR_Y(\theta)=\left[\begin{array}{cccc} 
1 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 \\
0 & 0 & \cos\frac{\theta}{2} & -\sin\frac{\theta}{2} \\
0 & 0 & \sin\frac{\theta}{2} & \cos\frac{\theta}{2} 
\end{array}\right]
\label{eq:cry}
\end{equation}

\begin{equation} 
\centering
CR_Z(\theta)=\left[\begin{array}{cccc} 
1 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 \\
0 & 0 & e^{\frac{i\theta}{2}} & 0 \\
0 & 0 & 0 & e^{\frac{i\theta}{2}} 
\end{array}\right]
\label{eq:crz}
\end{equation}

\subsection{Controlled Swap Gate}
Another type of controlled gate is the controlled SWAP gate. The SWAP gate measures the difference between two quantum states and outputs the result to an ancilla qubit. Therefore, this gate is a three-qubit gate. The SWAP test output values range from 0.5 to 1. Maximally different (orthogonal) states will measure 1 with 50\% probability while identical states will measure 1 with 100\% probability. The SWAP test gate can be used to measure quantum state fidelity. The controlled swap gate is described in Equations \ref{eq:cswap_eq} and \ref{eq:cswap_matrix}.



\begin{equation} 
\centering
CSWAP(q_{0},q_{1},q_{2})=|0\rangle \langle0|\otimes I \otimes I + |1\rangle \langle1| \otimes SWAP
\label{eq:cswap_eq}
\end{equation}

\begin{small}
\begin{equation} 
\centering
CSWAP(q_{0},q_{1},q_{2})=\left[\begin{array}{cccccccc} 
1 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\
0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\
0 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\\
\end{array}\right]
\label{eq:cswap_matrix}
\end{equation}
\end{small}



%Figure \ref{fig:swap_test} depicts a swap test being performed. The ancilla qubit, $q_0$, is placed is superposition using a Hadamard gate. Then a swap test is performed between $q_1$ and $q_2$ and measured onto $q_0$. Another Hadamard gate is performed on the ancilla qubit. Finally, the ancilla qubit is then measured onto a classical bit to obtain the result.


%\begin{figure}[ht]			% Add figure one
%	\centering
%	\includegraphics[width=0.7\linewidth]{figures/swap_test2.png}
 %   \caption{Swap Test Quantum Circuit}
  %  \label{fig:swap_test}
%\end{figure} 

One advantage of the CSWAP gate is that it only requires the measurement of the ancilla qubit. When qubits are measured directly, their states collapse and the superposition is lost. The Swap test allows the superposition of the other qubits to be maintained by measuring the quantum state fidelity through the ancilla qubit instead of measuring the qubits directly. Therefore, minimal information is lost through measurement.




\subsection{Quantum Entanglement}
Another key principle of quantum computing is quantum entanglement. A qubit’s state is said to be entangled when its measurement is dependent on the measurement of another qubit. This dependence allows information to be transferred between qubits, even if they are not physically close together (a phenomena sometimes referred to as "action at a distance"). When one entangled qubit is measured, the other entangled qubit's state also collapses. For example, if two qubits are entangled using the CNOT gate, after the state of one qubit is measured, the state of the second entangled qubit can be predicted with absolute certainty. Quantum entanglement is a key component of the quantum advantage over classical computing, as it is a property of quantum computing with no classical equivalent.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Grover's Algorithm}

In classical computing, the complexity of unstructured search is $O(N)$, where N is the size of the list being searched. Assume there is a list that have N elements. We want to find a special element in this list, and we check the element in list one by one. In the best case, we just need to check one element, and in the worst case, we need to check all elements. Therefore, we need to check $\frac{N}{{2}}$ elements on average. However, there is an algorithm called Grover's algorithm that can quadratically improve the speed of unstructured search in quantum computing. This algorithm was invented by Lov Grover in 1996. The complexity of Grover’s algorithm is $O(\sqrt{N})$.

Grover’s algorithm uses a black box function called oracle to solve the problem. This oracle is a diagonal matrix, and it can add a negative phase to the solution states. For example, we have two qubits and our target state is $|11\rangle$. Then, Our oracle $U_{t}$ will look like this:

\begin{equation}
    U_{t}=
    \begin{bmatrix}
    1&0&0&0\\
    0&1&0&0\\
    0&0&1&0\\
    0&0&0&-1
    \end{bmatrix}
\end{equation}

And for each state $|x\rangle$ in the list,
\begin{equation}
    U_{t}|x\rangle=
    \begin{cases}
          |x\rangle &  \text{for} \quad x\neq t\\
         -|x\rangle &  \text{for} \quad x= t\\
    \end{cases}  
\end{equation}

where $t$ is our target item $|11\rangle$.

Grover’s algorithm works with the amplitude amplification. It enhances the probability of measuring the target state. The amplitude amplification begins in a uniform superposition $|s\rangle$, which is constructed from $|s\rangle=H^{\otimes n}|0\rangle^n$ and can be expressed as $|s\rangle=\frac{1}{\sqrt{N}}\sum_{x=0}^{N-1}|x\rangle$. Using $|s\rangle, |s’\rangle$ and $|t\rangle$, we can calculate the reflection angle $\theta$. Assume vectors $|s’\rangle$ and $|t\rangle$ are perpendicular, we have $|s\rangle=sin\theta|t\rangle+cos\theta|s’\rangle$. Solving this function, the reflection angle $\theta$ can be represent as this form.~\citep{eleanor2011quantum}.

\begin{equation}
    \theta=arcsin\langle s|t\rangle=arcsin\frac{1}{\sqrt{N}}
\end{equation}

Next, we use the oracle reflection $U_f$ to reflect the state $|s\rangle$ across the $|s’\rangle$. This switches the amplitude in front of the $|t\rangle$ to negative. Then, we use another reflection $U_s$ on the state $|s\rangle$ where $U_s=2|s\rangle\langle s|-1$ to map the state to $U_sU_f|s\rangle$. These two reflections make the state $|s\rangle$ closer to the state $|t\rangle$ and decrease the amplitudes of the other states. We repeat these two steps n times. We will have the state $|\psi_n \rangle$, where $|\psi_n \rangle=(U_sU_f)^n |s\rangle$.~\citep{eleanor2011quantum}.




\subsection{Grover's Algorithm Example with 3 qubits}
In this case, we have $N=8$, so we need 3 qubits. The qubits we need for Grover’s algorithm can be calculated by $n=log_2N$. Our reflecting angle $\theta$ is:

\begin{equation}
    \theta=arcsin\frac{1}{\sqrt{8}}
\end{equation}

Let’s start with finding just one target state. Suppose we are looking for the state $|111\rangle$. First, we need to apply Hadamard gates to all the qubits, so we can switch all the qubits into superposition state and create a uniform superposition for all possible states in the list. 

\begin{equation}
    |\phi_{1}\rangle=\frac{1}{\sqrt{8}}(|000\rangle+|001\rangle+|010\rangle+|011\rangle+|100\rangle+|101\rangle+|110\rangle+|111\rangle)
\end{equation}

\begin{figure}[h]
    \centering
    \includegraphics[scale= 0.3]{figures/background/grover 1.png} 
    \caption{Grover circuit 1} \label{grover circuit 1}
\end{figure}

Then, we need to use the phase oracle to mark the target state. 

\begin{equation}
    |\phi_{2}\rangle=\frac{1}{\sqrt{8}}(|000\rangle+|001\rangle+|010\rangle+|011\rangle+|100\rangle+|101\rangle+|110\rangle-|111\rangle)
\end{equation}

\begin{figure}[h]
    \centering
    \includegraphics[scale= 0.3]{figures/background/grover 2.png} 
    \caption{Grover circuit 2} \label{grover circuit 2}
\end{figure}

Next, we need to apply the amplification circuit to the qubits. We follow these steps to create a amplification circuit. 
\begin{itemize}
    \item Apply the Hadamard gates and the Pauli X gates to all three qubits
    \item Apply a controlled Z gate with the control qubits $q_0$ and $q_1$ and the target qubit $q_2$ 
    \item Apply the Hadamard gates and the Pauli X gates to all three qubits again
\end{itemize}

\begin{figure}[h]
    \centering
    \includegraphics[scale= 0.3]{figures/background/grover 3.png} 
    \caption{Grover circuit 3} \label{grover circuit 3}
\end{figure}

Finally, we get the histogram of measuring the probability of our target state $|111\rangle$.

\begin{figure}[h]
    \centering
    \includegraphics[scale= 0.3]{figures/background/grover p.png} 
    \caption{Histogram of Measuring the probability} \label{grover p}
\end{figure}

Also, we can use Grover’s algorithm to find multiple target states in list. Grover’s algorithm can use the transformation of statevector to solve multiple targets problems. We initialize the statevector with all states in $|0\rangle$. We will switch the state $|0\rangle$ to state $|1\rangle$ if it is a target state.

For example, if our target state is $|000\rangle, |010\rangle$ and $|111\rangle$, the statevector transformation will be:

\begin{equation}
    [0,0,0,0,0,0,0,0] \rightarrow [1,0,1,0,0,0,0,1]
\end{equation}


==> sections/system.tex <==
\section{SYSTEM DESIGN}

%This chapter discusses the problem setting and system architecture of \sol~that includes its framework, design logic and functionalities of key modules.

%In \sol, we consider a given set of initial values as inputs, $\{v_1,...v_i...,v_n\} \in I$. For each value, it is associated with its index. Therefore, the data set container (index, value) pairs. Specified by the users, some of the values, $\{v_i,...v_j\} \in GS$, are defined as searching targets. The goal is to find the indexes of targets. Therefore, both indexes and values will be involved.

%We utilize Grover's search algorithm to complete the task. However, the original algorithm only amplifies the amplitude of the targeted states. It fails to determine and output the targets and indexes directly. Additionally, since both indexes and values need to be encoded, the qubit requirement is larger than value-only searches. Thus, our objective is to output the targeted (index, value ) pairs and reduce the number of required qubits.

This section presents the problem setting and system architecture of \soll, a quantum-classical system designed for searching targeted (index, value) pairs. The system receives a set of initial values, ${v_1,...v_i,...v_n} \in D$, each of which is associated with an index to form the (index, value) pairs. The set of targets, ${v_i,...v_j} \in T$, is specified by the users, and the objective is to find the corresponding indexes of the targets.

To achieve this goal, we utilize Grover's search algorithm, which is a well-known quantum algorithm for unstructured search problems. However, the original algorithm only amplifies the amplitude of the targeted states, and it does not directly output the targets and indexes. Moreover, since both the indexes and values need to be encoded, the qubit requirement is higher than that of value-only searches. Therefore, our objective is to output the targeted (index, value) pairs while reducing the number of required qubits.

To realize this objective, we propose a hybrid approach that combines quantum and classical computing resources. Specifically, the system consists of a quantum part and a classical part. The quantum part is responsible for implementing Grover's search algorithm to amplify the amplitude of the targeted states, and the classical part performs postprocessing to extract the (index, value) pairs.

\begin{figure*}[ht]
\centering
\includegraphics[width=0.75\linewidth]{figures/IQuSearch.pdf}
\caption{IQuSearch System Architecture}
\label{fig:system}
\end{figure*}

The hierarchical structure of \soll's system architecture is displayed in Figure \ref{fig:system}, which demonstrates a quantum-classical system design. Input data, such as unstructured databases, is submitted to the classical component and managed by the \textbf{Data Preprocessing} module. During this phase, the module analyzes the data's size, index ranges, and extracts metadata for subsequent processing.

The \textbf{Index/Value Management} module receives the processed data, with its functionalities divided into two scenarios. Algorithm~\ref{alg:SI} Storing Indexes, Algorithm~\ref{alg:RI} Restoring Indexes and Algorithm~\ref{alg:UV} Updating Values was implemented in this module. The details of these algorithms will describe in next section. In the first iteration scenario, the system employs its original index and value associations. In the following-up iteration scenario, the module regenerates new indexes and values after filtering out unlikely data points, as informed by the Quantum State Analyst module. In this case, the module must maintain a mapping between generated and original indexes/values to return the original values to clients.

The \textbf{Quantum Data Encoder} module accepts the processed data from the Index/Value Manager and encodes the classical data to quantum qubits. As the data changes every iteration, the encoding must be updated accordingly. The \textbf{Amplification Preparation} module calculates the number of amplitude amplifications, such as reflections, based on the iteration number and previous results. This number is used by the \textbf{Logical Circuit Generator} to prepare a logical circuit for quantum search.

This logical circuit is passed to a quantum computer, where Grover's search algorithm is conducted with a given number of amplitude amplification within the \textbf{Quantum Circuit Executor} module. The quantum states are measured by the \textbf{Quantum State Measurement} module and transferred back to the classical component for further processing at the end of the search.

Upon receiving the results, the {\bf Quantum State Analyst} module is activated to perform Algorithm~\ref{alg:F} Filter. If the algorithm finds all solutions, their original indexes will be returned. Otherwise, it conducts filtering to ensure that only potential solutions enter the next iteration. With this feature, the problem set is reduced when the Index/Value Management modules are called in the second and following rounds. Consequently, fewer qubits are required to continue the search. Meanwhile, the mappings between current and original indexes and values are maintained.
